ChemHTS: Hierarchical Tool Stacking for Enhancing Chemical Agents

Large Language Models (LLMs) have demonstrated remarkable potential in scientific research, particularly in chemistry-related tasks such as molecular design, reaction prediction, and property estimation. While tool-augmented LLMs have been introduced to enhance reasoning and computation in these domains, existing approaches suffer from tool invocation errors and lack effective collaboration among diverse tools, limiting their overall performance. To address these challenges, we propose ChemHTS (Chemical Hierarchical Tool Stacking), a novel method that optimizes tool invocation pathways through a hierarchical stacking strategy. ChemHTS consists of two key stages: tool self-stacking warmup and multi-layer decision optimization, enabling LLMs to refine tool usage dynamically. We evaluate ChemHTS across four classical chemistry tasks and demonstrate its superiority over strong baselines, including GPT-4o, DeepSeek-R1, and chemistry-specific models, including ChemDFM. Furthermore, we define four distinct tool-stacking behaviors to enhance interpretability, providing insights into the effectiveness of tool collaboration. Our dataset and code are publicly available at \url{https://github.com/Chang-pw/ChemHTS}.

==> 03background.tex <==
\subsection{Single Tool Invocation}
An LLM that depends on invoking a single tool to complete a task operates with fixed inputs and outputs, limiting its ability to dynamically adapt its workflow. This is exemplified in Algorithm.~\ref{tool stacking} with maxIter set to 1.


\subsection{Tool Stacking}
%工具堆叠（Tool Stacking）可以理解为在任务执行过程中，依次调用多个工具，并将前一个工具的输出作为下一个工具的输入，以逐步优化任务的执行效果。这种方法类似于多步推理（Multi-step Reasoning），在 LLM 任务执行过程中起到了类似流水线（Pipeline）的作用。
Tool stacking refers to the ability of LLMs to invoke multiple tools iteratively and integrate different tools at various levels, thereby optimizing task execution. This can be understood as sequentially invoking multiple tools during task processing as shown in Algorithm.~\ref{tool stacking}, where the output of one tool serves as the input for the next. This iterative process incrementally enhances task performance. 
\begin{algorithm}
\caption{Tool Stacking Execution}
\begin{algorithmic}[1]
\REQUIRE Input $I$, Tool Set $\{T_1, T_2, \dots, T_n\}$, Maximum Iterations $maxIter$
\ENSURE Final Output $O_{final}$
\STATE $O \gets I$
\STATE $iter \gets 0$
\WHILE{$iter < maxIter$}
    \STATE Model selects $T_r$ from $\{T_1, T_2, \dots, T_n\}$
    \STATE $O \gets T_r(O)$
    \STATE $iter \gets iter + 1$
\ENDWHILE
\STATE $O_{final} \gets O$
\RETURN $O_{final}$
\end{algorithmic}
\label{tool stacking}
\end{algorithm}




==> figures/algorithm.tex <==
\begin{algorithm}[H]
\caption{Self-stacking Tool Selection Algorithm}
\label{alg:tool_stacking}
\begin{algorithmic}[1]
\REQUIRE Chemical task $\mathcal{T}$, tool library $\mathcal{L}$, threshold for performance degradation $\epsilon$, parameter $m$ for Top-$m$ relevant tools selection, parameter $k$ for Top-$k$ tool combinations selection.
\ENSURE Optimal tool combinations for stacking.

\STATE \textbf{Step 1: Initial Tool Selection}
\STATE Select the m most relevant tools 
$\{Tool A_1, Tool A_2,...,Tool A_m\}$ from the tool library $\mathcal{L}$ based on their relevance to $\mathcal{T}$.

\STATE \textbf{Step 2: Preliminary Evaluation}
\STATE Evaluate the performance of a single tool ($Tool A_i$).
\STATE Evaluate the performance of the self-stacking configuration ($Tool A_i$ $\to$ $Tool A_i$).

\STATE \textbf{Step 3: Check for Performance Degradation}
\IF{Repeated invocations lead to performance degradation (difference $\geq \epsilon$)}
    \STATE Discontinue further stacking of the same tool type ($Tool A_i$).
\ENDIF

\STATE \textbf{Step 4: Top-$k$ Selection}
\STATE Identify the Top-$k$ most performant tool combinations from the evaluations for the next round of stacking. 

\end{algorithmic}
\end{algorithm}

\begin{algorithm}[htbp]
\caption{Stacking with Additional Tools Algorithm}
\label{alg:tool_stacking_step2}
\begin{algorithmic}[1]
\REQUIRE Top-$k$ optimal tool combinations, all available tools, maximum stacking depth $n$
\ENSURE Optimal execution trajectory
\STATE Initialize best\_trajectory $\gets$ None
\STATE Initialize best\_performance $\gets$ $-\infty$
\FOR{each combination in Top-$k$ optimal tool combinations}
    \STATE Initialize current\_stack $\gets$ combination
    \STATE Initialize depth $\gets$ 1
    \WHILE{depth $\leq$ $n$}
        \STATE Evaluate performance of current\_stack
        \IF{performance degrades}
            \STATE \textbf{break}
        \ENDIF
        \IF{current\_stack's performance $>$ best\_performance}
            \STATE best\_performance $\gets$ current\_stack's performance
            \STATE best\_trajectory $\gets$ current\_stack
        \ENDIF
        \FOR{each tool in all available tools}
            \STATE new\_stack $\gets$ current\_stack + tool
            \STATE Evaluate performance of new\_stack
            \IF{performance improves}
                \STATE current\_stack $\gets$ new\_stack
                \STATE \textbf{break}
            \ENDIF
        \ENDFOR
        \STATE depth $\gets$ depth + 1
    \ENDWHILE
\ENDFOR
\RETURN best\_trajectory
\end{algorithmic}
\end{algorithm}



==> tables/analysis3.tex <==



\setlength\tabcolsep{1pt}
%
\begin{table}[!htb]
    \centering
    \tiny
    \definecolor{lightgray}{gray}{0.9} % 定义浅灰色
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{ccccccccccc}
        \toprule
        \multirow{2}{*}{Tool Number} & \multicolumn{8}{c}{Train Data Number} & \multirow{2}{*}{AVG} \\ 
        \cmidrule(lr){2-9}
        & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{20} & \multicolumn{2}{c}{30} & \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        & NUM & BLEU-2 & NUM & BLEU-2 & NUM & BLEU-2 & NUM & BLEU-2 & \\
        \midrule
        2 & 0.6 & 0.79 & 2.7 & 0.89 & 3.0 & 0.89 & 3.2 & 0.87 & 0.86 \\
        3 & 0.4 & 0.81 & 2.5 & 0.87 & 2.8 & 0.86 & 3.0 & 0.85 & 0.85 \\
        4 & 0.6 & 0.80 & 2.8 & 0.88 & 3.0 & 0.87 & 3.2 & 0.86 & 0.86 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Details of the training and test sets for the four chemistry tasks.}
    \label{tab:analysis3}
\end{table}

